Enhancing Object Coherence in Layout-to-Image Synthesis

Layout-to-image synthesis is an emerging technique in conditional image generation. It aims to generate complex scenes, where users require fine control over the layout of the objects in a scene. However, it remains challenging to control the object coherence, including semantic coherence (e.g., the cat looks at the flowers or not) and physical coherence (e.g., the hand and the racket should not be misaligned). In this paper, we propose a novel diffusion model with effective global semantic fusion (GSF) and self-similarity feature enhancement modules to guide the object coherence for this task. For semantic coherence, we argue that the image caption contains rich information for defining the semantic relationship within the objects in the images. Instead of simply employing cross-attention between captions and latent images, which addresses the highly relevant layout restriction and semantic coherence requirement separately and thus leads to unsatisfying results shown in our experiments, we develop GSF to fuse the supervision from the layout restriction and semantic coherence requirement and exploit it to guide the image synthesis process. Moreover, to improve the physical coherence, we develop a Self-similarity Coherence Attention (SCA) module to explicitly integrate local contextual physical coherence relation into each pixel's generation process. Specifically, we adopt a self-similarity map to encode the physical coherence restrictions and employ it to extract coherent features from text embedding. Through visualization of our self-similarity map, we explore the essence of SCA, revealing that its effectiveness is not only in capturing reliable physical coherence patterns but also in enhancing complex texture generation. Extensive experiments demonstrate the superiority of our proposed method.

==> check_list.tex <==
\section{Reproducibility Checklist}
This paper:

Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)

Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)

Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)

Does this paper make theoretical contributions? (no)

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.

A motivation is given for why the experiments are conducted on the selected datasets (yes)

All novel datasets introduced in this paper are included in a data appendix. (NA)

All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)

All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)

Does this paper include computational experiments? (yes)

If yes, please complete the list below.

Any code required for pre-processing data is included in the appendix. (yes).

All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)

All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)

All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)

If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)

This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)

This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)

This paper states the number of algorithm runs used to compute each reported result. (yes)

Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (no)

The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)

This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)

This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)

==> figs/compare_complex_texture.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.73\linewidth]{figs/compare_complex_texture1.pdf}
    \caption{Qualitative comparison results with FreestyleNet on the generation of complex texture.}
    \label{fig:compare_complex_texture}
\end{figure*}

==> figs/compare_physical_coherence.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.73\linewidth]{figs/compare_physical_coherence1.pdf}
    \caption{Visual comparison results with FreestyleNet on the generation of physical coherence.}
    \label{fig:compare_physical_coherence}
\end{figure*}

==> figs/further_compare.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/further_compare1.pdf}
    \caption{Visual comparison results with FreestyleNet on the generation of complex texture and physical coherence.}
    \label{fig:further_compare}
\end{figure*}

==> figs/supply_semantic_coherence_problem.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/supply_semantic_coherence_problem1.pdf}
    \caption{\textcolor{red}{Supplementary to \cref{fig:problem}.} We present more cases of prevailing challenges of semantic coherence.}
    \label{fig:supply_semantic_coherence}
\end{figure*}
